Constrained Language Models Yield Few-Shot Semantic Parsers

We explore the use of large pretrained language models as few-shot semantic parsers. The goal in semantic parsing is to generate a structured meaning representation given a natural language input. However, language models are trained to generate natural language. To bridge the gap, we use language models to paraphrase inputs into a controlled sublanguage resembling English that can be automatically mapped to a target meaning representation. Our results demonstrate that with only a small amount of data and very little code to convert into English-like representations, our blueprint for rapidly bootstrapping semantic parsers leads to surprisingly effective performance on multiple community tasks, greatly exceeding baseline methods also trained on the same limited data.

==> abstract-fodder.tex <==




We consider how to rapidly develop a semantic parser, which translates natural language sentences into some structured meaning representation.  Our goal is to exploit a large pretrained language model (specifically fine-tuned GPT-2 or few-shot GPT-3), which can try to imitate \emph{examples} of translations.
Unfortunately, the language model excels more at analyzing the natural-language inputs than at generating structured outputs of a sort that did not appear in its pretraining data.
Since the model was pretrained on English, we ask it only to
translate (i.e., paraphrase) the input into a controlled sublanguage of English \cite{Marzoev:20} that can then be mechanically translated into the original structured target representation.
We demonstrate the benefits of this approach on several semantic parsing tasks, using few task-specific training examples yet obtaining reasonable top-1 and top-$k$ performance, especially with GPT-3.





We demonstrate that large autoregressive language models such as GPT-3 enable a new approach to the idea of casting semantic parsing as one of paraphrasing.%
Our proposal acknowledges the fact that such models are pretrained to generate \emph{language}, rather than some task-specific form: a minimal number of examples is sufficient to bootstrap an initial parser, given a  mapping between a target representation and a linguistic form closer to natural language.
Through experiments on multiple community datasets we show that few-shot GPT-3 and fine-tuned GPT-2 are more data efficient when mapping utterances to language-like representations, and that this can be further improved with explicit decoding constraints.  The performance of this approach with GPT-3, both at top-1 and small top-$k$ prediction, opens a new frontier of rapid semantic parser development. %

